Beyond Robustness: A Taxonomy of Approaches towards Resilient Multi-Robot Systems

Robustness is key to engineering, automation, and science as a whole. However, the property of robustness is often underpinned by costly requirements such as over-provisioning, known uncertainty and predictive models, and known adversaries. These conditions are idealistic, and often not satisfiable. Resilience on the other hand is the capability to endure unexpected disruptions, to recover swiftly from negative events, and bounce back to normality. In this survey article, we analyze how resilience is achieved in networks of agents and multi-robot systems that are able to overcome adversity by leveraging system-wide complementarity, diversity, and redundancy - often involving a reconfiguration of robotic capabilities to provide some key ability that was not present in the system a priori. As society increasingly depends on connected automated systems to provide key infrastructure services (e.g., logistics, transport, and precision agriculture), providing the means to achieving resilient multi-robot systems is paramount. By enumerating the consequences of a system that is not resilient (fragile), we argue that resilience must become a central engineering design consideration. Towards this goal, the community needs to gain clarity on how it is defined, measured, and maintained. We address these questions across foundational robotics domains, spanning perception, control, planning, and learning. One of our key contributions is a formal taxonomy of approaches, which also helps us discuss the defining factors and stressors for a resilient system. Finally, this survey article gives insight as to how resilience may be achieved. Importantly, we highlight open problems that remain to be tackled in order to reap the benefits of resilient robotic systems.

==> 041-perception-long.tex <==
%!TEX root = 00-main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Perception and Estimation}
\label{subsec:perception}
% Other names:
% Jon How
% Tokekar
% Alonso Mora
% \LC{state what the section covers}
% \LC{say something about relevance for applications (in particular: multi robot)}
% \fixit{Can the following paragraphs be clearer in terms of how the cited methods provide robustness / resilience?  How do they address uncertainty? Disruptions?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% RELEVANCE FOR MULTI ROBOT OPERATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Perception ---the robot’s ability to sense and understand the surrounding environment--- is a key enabler for autonomous systems’ operation in complex environments, and provides functionalities such as estimating the location of the robot, building a map of obstacles in its surroundings, detecting, classifying, and tracking objects. 
This capability is even more crucial for multi-robot systems, where a shared understanding of the world is 
 a key requirement for successful 
interaction. 

However, multi-robot systems pose new challenges to perception: 
(i) the sensor data is collected independently by multiple robots, possibly equipped with different sensor suites and with limited onboard compute, 
(ii) the team needs to form a shared world model in the face of communication constraints (\eg bandwidth, communication range, privacy), and (iii) the scale of multi-robot perception problems exacerbates 
the limitations that already arise in single-robot perception (\eg scalability, noisy and out-of-distribution measurements).

% Here we review a broad umbrella of perception problems 
% Spatial perception is a broad umbrella for challenges in state estimation and inference, computer vision and signal processing, and machine learning. 
In the following, we review perception problems arising in multi-robot systems, spanning several  
subdomains (\eg 
low-level perception and 2D vision,
localization and mapping,
% object tracking, 
and high-level scene understanding). 
Note that we restrict our focus to \emph{spatial} perception (\ie we are mainly concerned with estimating 
quantities that live in 3D space), and do not cover other perception problems (\eg action and emotion recognition) nor 
prediction problems.
% We also 
% discuss typical stressors,
% and classify existing work into 
% % We organize the review by classifugin  we highlight open problems across the 
% pre-operative, intra-operative, and post-operative approaches.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Pre-operative approaches.} We review pre-operative approaches for 
(i) low-level perception, (ii) localization, mapping, and estimation, and (iii) describe open problems in high-level
multi-robot learning and real-time scene understanding.

\subsubsection{Low-level Perception and 2D Vision}
Low-level perception focuses on image --or more generally sensor's signal-- processing and is typically finalized to 
detecting features or objects, performing pixel-wise semantic segmentation, 
and recognizing known places, among other problems. Low-level perception methods are often referred to as the \emph{perception front-end}~\cite{Cadena16tro-SLAMsurvey}. In these problems, common stressors include
illumination and viewpoint changes, presence of unexpected dynamic elements in the scene, and in general the presence of 
nuisances that are irrelevant for the perception task~\cite{Soatto14iclr}. 
The following approaches are classified as pre-operative since they do not adapt during operation, 
are often designed for the worst case, or do not explicitly deal with stressors.
% unknown and we try to get robustness against them, intraclass shape variations

Multi-robot research has extensively investigated \emph{distributed place recognition}, where 
robots in a team have to detect whether they are observing the same place; place recognition 
enables re-localization, and loop closure detection in Simultaneous Localization and Mapping (SLAM)~\cite{Cadena16tro-SLAMsurvey}. %~\cite{Lajoie20ral-doorSLAM}.
In a centralized setup, a common way to obtain loop closures is to use visual
place recognition methods, which compare compact image descriptors to find
potential loop closures. This is traditionally done with global visual
features~\cite{Oliva01ijcv,Ulrich00icra,Arandjelovic16cvpr-netvlad}, or local visual
features~\cite{Lowe99iccv,Bay06eccv} which can be quantized in a bag-of-word
model~\cite{Sivic03iccv}. The feature descriptors are designed to gain robustness 
to the stressors (\eg viewpoint changes). 
Distributed loop closure detection aims at detecting loop closures without exchanging raw data, 
a desirable feature when the robots operate under range and bandwidth constraints.
Tardioli~\etal~\cite{Tardioli15iros} use visual vocabulary indexes instead of descriptors to reduce the required bandwidth.
Cieslewski and Scaramuzza~\cite{Cieslewski18icra} propose distributed
and scalable solutions for place recognition in a fully connected team of
robots, using bag-of-words of visual features~\cite{Cieslewski17ral-bow} or 
full-image NETVLAD descriptors~\cite{Cieslewski17mrs-netvlad}. 
Tian~\etal~\cite{Tian18rss,Tian19arxiv}, Lajoie~\etal~\cite{Lajoie20ral-doorSLAM}, and
Giamou~\etal~\cite{Giamou18icra} propose approaches to coordinate the
data exchange during the geometric verification step.
%, accounting for the availablecommunication and computation resources.

Recent effort in computer vision has focused on \emph{segmentation and recognition problems}.
Liu~\etal~\cite{Liu20cvpr-when2com,Liu20arxiv-who2com} learn to construct
communication groups and decide when to communicate to complete
multi-agent semantic segmentation and 3D shape recognition tasks. 
% auction-based methods: % no: this is for camera control
% Yiming Li, Bir Bhanu, and Wei Lin. Auction protocol for
% camera active control. In Proceedings of the IEEE International
% Conference on Image Processing (ICIP), pages 4325–
% 4328. IEEE, 2010.
% Faisal Qureshi and Demetri Terzopoulos. Smart camera
% networks in virtual reality. Proceedings of the IEEE,
% 96(10):1640–1656, 2008.
 Reinartz~\etal~\cite{Reinartz13cg-distributedRecognition} 
 develop a multi-agent object recognition system based on satellite imagery.
Wu~\etal~\cite{Wu19iccv-RLVideoRecognition} use multi-agent reinforcement learning to 
sample frames that maximize the accuracy of video recognition.
Mousavi~\etal~\cite{Mousavi19iros-multiAgentImageClassification} propose 
a  multi-agent image classification approach based on RL and generalized policy gradient.
Male\v{s}~\etal~\cite{Males19esa-multiAgentFaceTracking} propose a hierarchical architecture for
multi-agent face tracking in video sequences.
Earlier work has focused on distributed object detection, including work on 
linear support vector machines~\cite{Pang14tc-distributedSVM}; in this case the goal is to parallelize the 
computation to speed up processing.

Low-level perception problems are often performed using learning-based techniques, including 
descriptor learning~\cite{Choy19iccv-FCGF,Sarlin20cvpr-superglue} and place recognition~\cite{Arandjelovic16cvpr-netvlad}.
While currently less used in robotics, the growing field of \emph{federated learning} investigates how to train machine learning models in a distributed fashion, with the goal of preserving privacy of the agents 
in the team and sharing computational resources~\cite{Yang19acm-federatedML,McMahan17aistats-federatedML,Konecny16arxiv-federatedML,Konecny18iclr-federatedML}.
This field is still in its infancy, with recent effort being devoted to dealing with unreliable agents~\cite{Li17arxiv-federatedML} and unreliable connectivity among agents~\cite{Salehi21toc-federatedML}. 
While most approaches listed in this section do not formally address the presence of stressors, the 
literature on \emph{adversarial learning}~\cite{Madry17arxiv-adversarialML} attempts to quantify and improve the robustness of a neural network to {perturbations}~\cite{Bastani16nips-robustNN,Cheng17springer-maximum,huang17iccav-safety,Kolter17icml-provableDefense,Pei17-DeepXplore,Ma18ieee-deepgauge,Dvijotham18-dual_approach_verification,Wong18neurips-provableDefense}.
Most of these approaches consider simple perturbations (\eg additive pixel-wise noise on an image) that lead the network to produce incorrect classification results. 
% \emph{Federated learning} has been recently proposed as a paradigm to distribute computation across multiple devices, while preserving privacy (\eg avoiding the exchange of raw data in favor of less sensitive information, such as model parameters). 
% both horizontal, vertical, and hybrid federated learning
% Federated learning is a recently proposed distributed machine learning paradigm for privacy preservation, which has found a wide range of applications where data privacy is of primary concern

\subsubsection{Localization, Mapping, and Estimation} 
Here we briefly review distributed estimation techniques and then focus on their applications in multi-robot teams. 
Estimation techniques typically constitute the \emph{perception back-end}~\cite{Cadena16tro-SLAMsurvey}, in that 
they take intermediate representations produced by low-level perception processes (the perception front-end) 
and use them to estimate the state of the system (\eg the pose of the robots, the 3D location and velocity of 
objects in the environment). 
In these problems, typical stressors include measurement noise, out-of-distribution data (typically produced by incorrect processing at the front-end or by off-nominal sensor behavior), as well as intermittent communication. 

Early work focuses on estimation with Gaussian noise, a setup that builds on well-established estimation-theoretic methods~\cite{Mendel95book,Dellaert17fnt-factorGraph} for which efficient solvers are now available (\eg~\cite{gtsam,Agarwal12-ceres}).
Distributed estimation in multi-agent systems has been also extensively investigated in robotics and 
sensor networks, with the goal of developing methods that converge to optimal estimates while only requiring local 
communication~\cite{Garin10ncs-surveyDistributedEstimation,Carli08jsac-distributedKF,Barooah07csm} 
and are possibly robust to unreliable communication channels~\cite{Schenato07ieee,Sinopoli04tac-KFintermittent,Schenato08tac}. 
%For the case of Gaussian measurement noise, 
Multi-robot research 
investigates multi-robot localization with different estimation
techniques, including Extended Kalman filters~\cite{Roumeliotis02tra,Zhou06iros}, 
information filters~\cite{Thrun03isrr}, and particle filters~\cite{Howard06ieee,Carlone10jirs-multiRobotSLAM}.
Maximum a posteriori and maximum likelihood estimation have recently been
adopted as a general and accurate framework for robotics; in SLAM problems, 
these frameworks lead to well-studied optimization problems, including \emph{pose graph optimization} (PGO)~\cite{Cadena16tro-SLAMsurvey} or \emph{factor graph optimization}~\cite{Dellaert17fnt-factorGraph}.
Early literature on multi-robot PGO focused on centralized approaches, where measurements 
are collected at a central station, which computes the trajectory estimates for all the
robots~\cite{Andersson08icra,Kim10icra,Bailey11icra,Lazaro11icra,Dong15icra}.
{Since the computation workload and the communication bandwidth of a
centralized approach grow with the number of robots, related work has 
explored \emph{distributed techniques}, in which robots perform local communication and share
the computational workload~\cite{Aragues11icra-distributedLocalization,Cunningham10iros,Cunningham13icra,Choudhary17ijrr-distributedPGO3D,tian_Asynchronous_2020,Tian19arxiv-distributedSEsync}; these techniques leverage problem structure and distributed optimization methods
to obtain optimal estimates from partial information exchange. % across the robots.

Recent work on multi-robot localization, mapping, and estimation has focused on 
the realistic case where some of the measurements used by the back-end are \emph{outliers}
(\ie they are affected by severe unmodeled noise). 
The fundamental problem of robust estimation has a long history and there are 
well established frameworks to model estimation problems with outliers, including 
M-estimation~\cite{Huber81} and consensus 
maximization~\cite{Chin18ECCV-robustFitting,Chin17slcv-maximumConsensusAdvances}. 
However, these frameworks typically lead to hard optimization 
problems~\cite{Chin18ECCV-robustFitting,Antonante21tro-outlierRobustEstimation}, and developing 
fast and effective solvers is still an active research area~\cite{Yang20neurips-certifiablePerception,Yang20ral-GNC,Barron19cvpr-generalAdaptiveLoss,Chebrolu2020arxiv-adaptiveRobustKernels}.
We remark that these approaches are still pre-operative (according to Definition~\ref{def:pre-operative}): for instance
M-estimators can be understood as maximum-likelihood estimators over heavy-tailed (but known) noise models.
Robust estimation is particularly important in multi-robot localization and mapping where 
incorrect measurements among the robots are more difficult to detect when the robots do not share a common reference frame.
Centralized outlier rejection techniques for multi-robot SLAM include 
voting schemes~\cite{Indelman14icra} and graph-theoretic methods~\cite{Mangelson18icra}; 
the Pairwise Consistency Maximization approach of~\cite{Mangelson18icra} has been particularly successful, has 
also been implemented in~\cite{Ebadi20icra-LAMP}, and is
 amenable for a distributed implementation~\cite{Lajoie20ral-doorSLAM,Chang21icra-KimeraMulti}. 
More recently, Tian~\etal~\cite{Tian21arxiv-KimeraMulti} propose a distributed M-estimation approach based on graduated non-convexity~\cite{Yang20ral-GNC} which is shown to lead to more accurate trajectory and map estimates.

% stressor: out of distribution measurements (Kimera-Multi, GNC), 
% sensor disruption (LAMP) - 
% intro
% copied from [FRANK R. HAMPEL, 1971]:
% ``The setup of robust estimation can be described
%  as follows (compare Hampel (1968); for the background, see Tukey (1960), Huber
%  (1964), (1968a), among others). We assume that the process generating the observa-
%  tions under consideration can approximately be described by some parametric
%  model (e.g. the model of independently and identically normally distributed obser-
%  vations), and we want to estimate the parameters of this model (or some function
%  of them), i.e. we want to find a statistic whose distribution is close to these para-
%  meter values. However, we know that the parametric model is not quite true;
%  and therefore we require that the distribution of the estimator changes only slightly
%  if the distribution of the observations is slightly altered from that of the strict para-
%  metric model with certain parameter values. (In order that this be possible one has
%  to presuppose a certain smoothness or "robustness" of the parametric model itself.)
%  We now have to specify the types of deviations to be allowed for.''
% \subsubsection{Object Tracking}
% object/people detection/tracking 
% Pol Rosello and Mykel J Kochenderfer. 2018. Multi-Agent Reinforcement Learning for Multi-Object Tracking. (2018), 1397--1404.

\begin{openProblem}[Learning in teams] \label{op:team_learning}
% keywords = {domain: perception, approach: pre-operative, interaction: cooperation, stressor: untargeter/targeted, out-of-distribution}
Federated and adversarial learning have the potential to enhance multi-robot operation 
but have found limited use in robotics.
Open challenges in federated learning for multi-robot systems include improving
communication bandwidth, energy efficiency, and security~\cite{Yu21arxiv-federatedML}. 
Regarding adversarial learning, robotics and computer vision applications 
require going beyond simple additive perturbation models, which are 
not well-suited to capture nuisances arising in real perception problems~\cite{Poursaeed18cvpr-adversarialML}.
\end{openProblem}

\begin{openProblem} [Distributed real-time scene understanding]
\label{op:scene_understanding}
% keywords = {domain: perception, approach: pre-operative, interaction: cooperation/collaboration, stressor: untargeted, out-of-distribution}
While multi-robot SLAM can be considered a mature field of research, the goal of achieving human-level 
understanding of the environment is still out of reach for a robot. 
Despite the growing literature on single-robot metric-semantic understanding~\cite{Rosinol20icra-Kimera,Salas-Moreno13cvpr,McCormac17icra-semanticFusion,Tateno15iros-metricSemantic,McCormac183dv-fusion++,Runz17icra-cofusion,Xu19icra-midFusion,Wald18ral-metricSemantic,Narita19arxiv-metricSemantic,Grinvald19ral-voxbloxpp,Tateno17cvpr-CNN-SLAM,Lianos18eccv-VSO,Behley19iccv-semanticKitti,Bowman17icra} and 
3D scene graph representations~\cite{Rosinol20rss-dynamicSceneGraphs,Armeni19iccv-3DsceneGraphs}, 
few papers have considered metric-semantic multi-robot mapping~\cite{Chang21icra-KimeraMulti,Tian21arxiv-KimeraMulti,Tchuiev20ral-semanticMultiRobotMapping,Yue20iros-semanticMultiRobotMapping}. 
%, with~\cite{Chang21icra-KimeraMulti} being the first work considering distributed dense metric-semantic mapping. 
Infusing semantic and high-level understanding in localization and mapping problems creates novel opportunities to 
improve resilience since a team of robots can dynamically adjust depending on the external context or the semantic 
elements in the scene (\eg presence of a threat).  
% distributed high-level understanding
% -- fully distributed architectures: communication interfaces
% Elizabeth Bondi. 2019. Bridging the Gap Between High-Level Reasoning in Strategic Agent Coordination and Low-Level Agent Development. (2019), 2402--2404.
%% METRIC SEMANTIC MAPPING
\end{openProblem}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Intra-operative approaches.} 
The literature on intra-operative approaches to perception is more sparse but growing.

\subsubsection{Low-level Perception and 2D Vision}
Learning-based approaches for low-level perception (\eg object detection) are challenged by 
(i) a potential shift between the training and testing distributions, and (ii) test instances 
that belong to the tails of the distribution (\eg rare examples) for which little training data is available.
Intra-operative approaches include methods that deal with these challenges online during operation. 
% while we will discuss domain adaptation and tran
% Online learning methods are receiving an increasing amount of attention, but still finds limited applications in multi-robot systems. 
Kalal~\etal~\cite{Kalal12pami-onlineLearningDetection} and
Prasad~\etal~\cite{Prasad18pcs-onlineLearningDetection} investigate online learning 
to detect and track objects in videos.
 The survey by Abass~\etal~\cite{Abbass20vc-onlineLearningTracking} provides a more extensive review of 
 online learning for visual tracking. 
 %Online learning currently finds limited applications in multi-robot systems. 

Recent work in robotics and autonomous vehicles uses learning-based methods to detect out-of-distribution 
examples online during operation.
%The line of work that is mosr related to our proposal is the one focusing on learning-based monitoring of neural networks
% Hecker\setal~\cite{Hecker18iv-failure} create a pipeline to predict whether an autonomous driving system will make bad 
% predictions in the future. 
% Saxena\setal~\cite{Saxena17} and Daftry\setal~\cite{Daftry16iros-introspective} develop a network to verify
%  collision-free trajectories for a vision-based drone platform. 
 Rahman~\etal~\cite{RahmanIROS19-falseNegative} process the hidden layer outputs of a neural 
 network to predict when a traffic sign detection network outputs false negatives. 
% Our work builds on previous learning methods for network monitoring by developing a model architecture and losses for 3D Mesh verification applying the network to 
% prune out bad predictions.
 Cheng~\etal~\cite{Cheng18date} and Henzinger~\etal~\cite{Henzinger20ecai} observe neuron activation patterns to monitor when the network is operating on inputs unlike the data seen during training.
  Hendrycks~\etal~\cite{Hendrycks16iclr} develop a method of monitoring network confidence based on softmax probabilities. Gupta and Carlone~\cite{Gupta20itsc-atom} propose
  Adversarially-Trained Online Monitor (ATOM) to detect incorrect detections of pedestrians in self-driving applications.
System-level monitoring approach are studied in~\cite{Antonante20tr-perSysMonitoring2} to detect off-nominal behaviors of perception modules.

\subsubsection{Localization, Mapping, and Estimation} 
We start by remarking that several approaches for robust estimation admit an alternative interpretation 
as intra-operative approaches. For instance, approaches based on graduated non-convexity, reweighted least squares, 
and dynamic covariance scaling~\cite{Yang20ral-GNC,Antonante21tro-outlierRobustEstimation,Sunderhauf13icra,Agarwal13icra} 
can be understood as approaches to adjust the measurement covariances (a key stressor variable, see Table~\ref{fig:key_var}) online, to down-weight out-of-distribution measurements. The connection between robust estimation and measurement weighting is a well-understood one and goes back to the seminal work from Black and Rangarajan~\cite{Black96ijcv-unification}, with more recent multi-robot applications in~\cite{Tian21arxiv-KimeraMulti}.
% Loc and map and estimation:
% - stressor: out of distribution measurements (Kimera-Multi, GNC), sensor disruption (LAMP) - can be just considered a different noise distribution
% - intra-operative: some approaches can be understood as can be understood as adaptation of covariances (black-rangarajan duality, GNC) but still assume inlier noise to be known

More recent work on robust estimation for robust localization, mapping, and learning goes further and 
explicitly tackles online adaptation. Antonante~\etal~\cite{Antonante21tro-outlierRobustEstimation} propose minimally tuned robust estimation algorithms that can learn the inlier noise statistics online. 
Barron~\cite{Barron19cvpr-generalAdaptiveLoss} and Chebrolu~\etal~\cite{Chebrolu2020arxiv-adaptiveRobustKernels} 
adjust the choice of robust loss function (within a parametric family) using an automatic online tuning procedure.

Other potential stressors include sensor mis-calibrations and sensor failures.
 Online calibration has been extensively investigated in the context of 
 kinematic odometry~\cite{Roy99icra-onlineCalibration}, 
  visual-inertial~\cite{Lee20iros-onlineCalibration,Geneva20icra-openVINS} and lidar-inertial odometry~\cite{Tagliabue20iser-lion}, 
 and SLAM~\cite{Nobre17iser-selfCalibration}.
 System-integration efforts have also investigated system reconfiguration in response to sensor 
 failures~\cite{Palieri21ral-locus}. A general framework for sensor selection based on resilient submodular maximization is investigated in~\cite{Tzoumas18cdc}.

\begin{openProblem}[Resilience and reasoning over failures]
\label{op:failure_reasoning}
% keywords = {domain: perception, approach: intra-operative, interaction: cooperation, stressor: targeted, out-of-distribution}
At the algorithmic level, resilient perception is still in its infancy: most perception frameworks 
are ``rigid'' and target robustness rather resilience and online adaptability. 
 It is desirable for future perception algorithms to perform automatic parameter tuning to adjust to 
 heterogeneous environmental conditions.
At the system level, monitoring of perception systems is also a largely unexplored topic: how to detect failures 
of perception algorithms? how to detect that the world models built by different robots in a team 
are inconsistent with each other? 
% perception monitoring
% need to reason over failures - online learning
% lack of tools to enable resilience/adaptation over time
More importantly, robot perception currently aims at \emph{detecting and isolating} off-nominal data (\eg outliers, sensor failures, 
algorithmic failures) rather than reasoning on the cause of those failures and learning how to avoid them in the 
future.
\end{openProblem}

\begin{openProblem} [Task-dependent perception and active perception]
\label{op:active_perception}
% keywords = {domain: perception, approach: intra-operative, interaction: cooperation/collaboration, stressor: untargeted, out-of-distribution}
As already stressed in~\cite{Cadena16tro-SLAMsurvey}, an open-challenge is to develop a tractable
and general framework for \emph{task-driven perception}, which can guide sensing and perception processes to 
maximize a task-driven performance metric (\eg obstacle avoidance) while minimizing computation, sensing, or communication. This is particularly important in multi-robot teams, where --under communication constraints-- it is desired for the robots to exchange the minimum amount of information to guarantee successful completion of a task.
 Conversely, resilience also requires active perception, \ie how to actively plan and control the robot to 
 minimize the impact of environmental stressors.
\end{openProblem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\textbf{Post-operative approaches.}
Postoperative approaches use batch training data collected by a robot over multiple deployments to identify stressors. 
% Note that learning-based approaches may also be pre-operative: for instance, a neural network 
% trained to perform object detection is designed to estimate the variable of interest ($x$ in Definition~\ref{def:pre-operative}) 
% in the face of given stressors ($\stressors$) in the training data.
% Instead post-operative approaches are explicitly design to identity over stressors.
% localization/mapping/estimation: system id methods and calibration. 
Approaches for offline system identification and sensor calibration fall in this category, 
see, \eg~\cite{Furgale13iros,Rehder16icra-extending}; in this case, the training is often augmented with external sensors (\eg a vicon system) to increase the observability of the resulting parameter estimation problem. 

More recently, post-operative approaches have focused on learning-based methods that can improve and adapt after multiple 
executions. In this sense, post-operative approaches are related to \emph{domain adaptation and transfer learning} in machine learning, where the goal is to allow a network --trained on a given training distribution-- to transfer to a different test distribution. 
The surveys~\cite{Zhuang19arxiv-domainAdaptation,Wang18neurocomputing-domainAdaptation} 
cover techniques for domain adaptation and perception applications including 
image classification, face recognition, semantic segmentation, and object detection. 
Domain adaptation can rely on external supervision, but can also be semi-supervised or unsupervised.

For future operation of multi-robot teams, the unsupervised setup is particularly appealing since 
it avoids massive human annotations~\cite{Jing20pami-selfsupervised}. 
The unsupervised (or self-supervised) setup relies on automatically generated labels 
produced by image generation techniques~\cite{Ledig17cvpr-superresolutionGAN}, 
classical vision algorithms~\cite{Li16cvpr-unsupervisedEdges,Jiang18eccv-selfsupervisedDepth}, 
or simulation~\cite{Dosovitskiy17arxiv-carla,Richter17iccv}. 
Self-supervision has been proven useful to learn depth~\cite{Wang18cvpr-selfsupervisedDepth,Godard19iccv-selfsupervisedDepth},
 optical flow~\cite{Liu19cvpr-selflow}, 
 visual odometry~\cite{Zhou17cvpr-selfsupervisedDepth, Yang20cvpr-D3VO}, 
 and feature descriptors for scan matching~\cite{Yew18eccv-3dfeatnet, Choy19iccv-FCGF, Bai20cvpr-D3Feat}. 
 % These tasks rely on the supervision from camera poses or relative rigid transformations for image warping and correspondence generation, and thus benefit from well-established  SLAM~\cite{Mur-Artal17tro-ORBSLAM2}, 3D reconstruction~\cite{Zhou18arxiv-open3D}, and SfM~\cite{Schonberger16cvpr-SfMRevisited} pipelines. Although these systems are off-the-shelf, they usually require long execution times, delicate parameter tuning, and human supervision to safeguard their correctness. 
In this landscape, \emph{self-training} methods start from a pre-trained model (using manual labels) and then 
build a larger dataset by automatically building \textit{pseudo-labels}
for a larger body of unlabeled data~\cite{Lee13icmlws-pseudolabel,Xie20cvpr-selftraining,Zoph20arxiv-selftraining,Wei20arxiv-selftraining,Yang21cvpr-sgp}.

\begin{openProblem}[Tuning and reconfiguration]
\label{op:tuning_reconfig}
% keywords = {domain: perception, approach: post-operative, interaction: cooperation/collaboration, stressor: targeted/untargeted, out-of-distribution}
While offline calibration is well understood, currently there are no efficient and automatic ways  
to automatically tune parameters and potentially reconfigure components in complex perception pipelines.
For instance, modern SLAM and VIO pipelines include tens to hundreds of tunable configuration parameters (\eg number of features, 
type of feature descriptors, etc.) that impact performance, 
are scenario-dependent, and rely on manual tuning from an expert. 
The large number of parameters (and the potential lack of ground-truth information) quickly makes brute-force and black-box 
approaches for tuning (\eg Bayesian optimization) impractical. 
This adds to the combinatorial complexity of choosing how to combine different algorithmic blocks comprising the robot 
perception system: which object detector? which 3D object pose estimation and tracking approach? which SLAM pipeline?   
% offline recalibration, parameter tuning and pipeline autoconfiguration
\end{openProblem}



==> 041-perception-notes.tex <==

%% BEST STORY:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Pre-operative approaches.}
% \LC{I suggest giving examples of what $x$ and $\phi$ are here}
% Low-level perception (focus on things not based on learning): 
% - detection and tracking/matching of primitieves (points, lines, planes)
% - 2D object detection
% - stressor: illumination and viewpoint changes, dynamic elements in the scene (Varun, Pablo): unknown and we try to get robustness against them, intraclass shape variations
% - why pre-operative: plan for worst case? no adaptation?
% - adversarial learning formalizes bounds
% - federated learning

% Loc and map and estimation:
% - stressor: noise
% - why pre-operative: distribution is known, no adaptation

% - stressor: disruption in communication
% - schenato etc.

% Loc and map and estimation:
% - stressor: out of distribution measurements (Kimera-Multi, GNC), sensor disruption (LAMP) - can be just considered a different noise distribution
% - why intra-operative: figure out outliers from inliers, detect sensor disruption, can be understood as adaptation of covariances

% \begin{openProblem}
% Limitations: bounds are unrelalistic (adversarial learning) or not formalized
%  - adversarial and federated learning
% distributed high-level understanding
% -- fully distributed architectures: communication interfaces
% task-dependent perception: communicate only what you need (stressor is computation and communication)
% \end{openProblem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Intra-operative approaches.}
% Loc and map and estimation:
% - stressor: out of distribution measurements (Kimera-Multi, GNC), sensor disruption (LAMP) - can be just considered a different noise distribution
% - intra-operative: some approaches can be understood as can be understood as adaptation of covariances (black-rangarajan duality, GNC) but still assume inlier noise to be known

% - step further more recent work on minimally tuned and Cyrill ()

% stressor: sensor miscalibration
% solution: online calibration

% Robust target tracking and pose/shape estimation
% - same as before.

% \begin{openProblem}
% perception monitoring
% need to reason over failures 
% lack of tools to enable resilience/adaptation over time
% \end{openProblem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\textbf{Post-operative approaches.}

localization/mapping/estimation: system id methods and calibration. 

low-level perception: Monitoring methods? Arjun? Niko?

selfsupervision: robot autonomously adapts instead of supervised where human designs

% tracking: 
% high-level understanding:

\begin{openProblem}
offline recalibration, parameter tuning and pipeline autoconfiguration
\end{openProblem}




%% ALTERNATIVE STORY:

\textbf{Pre-operative approaches.}
% \LC{I suggest giving examples of what $x$ and $\phi$ are here}
Low-level perception (focus on things not based on learning): 
- stressor: illumination and viewpoint changes, dynamic elements in the scene (Varun, Pablo)
- why pre-operative: plan for worst case? no adaptation? still deals with outliers

Loc and map and estimation:
- stressor: noise
- why pre-operative: distribution is known

- stressor: out of distribution measurements (Kimera-Multi, GNC), sensor disruption (LAMP)
- why intra-operative: figure out outliers from inliers, detect sensor disruption

\begin{openProblem}
distributed high-level understanding
task-dependent perception: communicate only what you need
\end{openProblem}

\textbf{Intra-operative approaches.}
Loc and map and estimation:
- more recent work on minimally tuned and Cyrill

\begin{openProblem}
perception monitoring
lack of tools to enable resilience/adaptation over time
\end{openProblem}

\textbf{Post-operative approaches.}
Learning-based approaches
- stressor: broad range, from the ones mentioned in pre-operative section 
- why post-operative: given x, figure out distribution of data

\begin{openProblem}
need to reason over failures 
\end{openProblem}

==> 06-conclusion.tex <==
%!TEX root = 00-main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                                                                        %%%%
%%%%                         SECTION : Conclusions                          %%%%
%%%%                                                                        %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

